Multicompartment Magnetic Resonance Fingerprinting

Magnetic resonance fingerprinting (MRF) is a technique for quantitative estimation of spin-relaxation parameters from magnetic-resonance data. Most current MRF approaches assume that only one tissue is present in each voxel, which neglects the tissue's microstructure, and may lead to artifacts in the recovered parameter maps at boundaries between tissues. In this work, we propose a multicompartment MRF model that accounts for the presence of multiple tissues per voxel. The model is fit to the data by iteratively solving a sparse linear inverse problem at each voxel, in order to express the magnetization signal as a linear combination of a few fingerprints in the precomputed dictionary. Thresholding-based methods commonly used for sparse recovery and compressed sensing do not perform well in this setting due to the high local coherence of the dictionary. Instead, we solve this challenging sparse-recovery problem by applying reweighted-l1-norm regularization, implemented using an efficient interior-point method. The proposed approach is validated with simulated data at different noise levels and undersampling factors, as well as with a controlled phantom imaging experiment on a clinical magnetic-resonance system.

==> macros_2.tex <==
\usepackage{fullpage,amsfonts,amsmath,amssymb,amsthm,bm,xspace,thmtools,thm-restate,asymptote,mathrsfs,appendix,array, comment}
\usepackage{multirow,graphicx, algorithm,algorithmic,caption,subcaption,url,cite,float}
\usepackage{mathtools}
%\hypersetup{colorlinks=true}
%\usepackage{hyperref}
\usepackage[colorlinks=true,urlcolor=blue,citecolor=blue]{hyperref}
\usepackage{todonotes}
\usepackage{array} 
\usepackage[noabbrev]{cleveref}
\usepackage{listings}
\lstset{language=Mathematica,columns=fullflexible,keywordstyle=\itshape}
\usepackage{xpatch}
\usepackage{thmtools}
\usepackage{apptools}

\makeatletter
\xpatchcmd{\thmt@restatable}{\csname #2\@xa\endcsname\ifx\@nx#1\@nx\else[{#1}]\fi}%
{\IfAppendix{\csname #2\@xa\endcsname}{\csname #2\@xa\endcsname[{#1}]}}
\makeatother

\newcolumntype{C}{ >{\centering\arraybackslash} m{7cm} }
\newcolumntype{D}{ >{\centering\arraybackslash} m{2cm} }
\newcolumntype{E}{ >{\centering\arraybackslash} m{1.5cm} }
\newcolumntype{F}{ >{\centering\arraybackslash} m{8.3cm} }
\newcolumntype{G}{ >{\centering\arraybackslash} m{8cm} }

\newcommand{\alignmulticolumn}[1]{\omit\rlap{$\displaystyle{#1}$}}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{theoremschema}[theorem]{Theorem Schema}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{method}[theorem]{Algorithm}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}

\def \endprf{\hfill {\vrule height6pt width6pt depth0pt}\medskip}

\numberwithin{equation}{section}

\newcommand{\smo}[1]{#1^{\downarrow}_\infty}
\newcommand{\mo}[1]{#1^{\downarrow}}
\newcommand{\sym}[1]{#1_\infty}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\Max}{Max}

\newcommand{\EV}{\text{even}}
\newcommand{\OD}{\text{odd}}


%Sparse noise constants
\newcommand{\wid}{\tau}
\newcommand{\DeltaG}{3.751}
\newcommand{\DeltaR}{5.056}
\newcommand{\botwid}{0.065}
\newcommand{\topwid}{0.2375}
\newcommand{\botwidG}{\botwid}
\newcommand{\topwidG}{\topwid}
\newcommand{\botwidR}{0.0775}
\newcommand{\topwidR}{0.165}
\newcommand{\etaG}{1.08732}
\newcommand{\etaR}{1.12597}
\newcommand{\psiG}{\etaG}
\newcommand{\psiR}{\etaR}
\newcommand{\zetaG}{0.087317}
\newcommand{\zetaR}{0.12597}
\newcommand{\betaG}{0.118824}
\newcommand{\betaR}{0.261070}
\newcommand{\alphaG}{1.09206}
\newcommand{\alphaR}{1.12633}
\newcommand{\alphajG}{0.907937}
\newcommand{\alphajR}{0.873678}
\newcommand{\QsiG}{1.39862}
\newcommand{\QsiR}{1.19352}
\newcommand{\waveG}{1.83193}
\newcommand{\waveR}{1.14055}


\newcommand{\KG}{K^{\mathcal{G}}}
\newcommand{\KR}{K^{\mathcal{R}}}
\newcommand{\DG}{D^{\mathcal{G}}}
\newcommand{\DR}{D^{\mathcal{R}}}

\newcommand{\wt}[1]{\widetilde{ #1 } }
\newcommand{\wh}[1]{\widehat{ #1 } }
\newcommand{\A}{\mathcal{A}}
\newcommand{\TV}{\mathrm{TV}}
\newcommand{\LB}{\mathrm{LB}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\CCC}{\mathcal{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\BB}{\mathcal{B}}
\newcommand{\DBB}{\mathcal{B}^{\brac{1}}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\bxi}{\bar{\xi}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\Noi}{\cN}
\newcommand{\sB}{\mathscr{B}}
\newcommand{\sV}{\mathscr{V}}
\newcommand{\sD}{\mathscr{D}}
\newcommand{\WW}{\mathcal{W}}
\newcommand{\DWW}{\mathcal{W}^{\brac{1}}}
\newcommand{\sW}{\mathscr{W}}
\newcommand{\II}{\mathcal{I}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\ZZ}{\mathbb{Z}}
\renewcommand{\Pr}{\mathbb{P}}
\renewcommand{\r}{\mathrm{r}}
\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}
\newcommand{\qj}{q(j)}
\newcommand{\Qaux}{Q_{\text{aux}}}
\newcommand{\QI}{Q_{\ml{I}}}
\newcommand{\QC}{Q_{\ml{C}}}
\newcommand{\RQ}{R}
\newcommand{\IS}{\ml{I}}
\newcommand{\CS}{\ml{C}}
\newcommand{\RC}{R_{C}}
\newcommand{\nearNoise}{\eta}

\newcommand{\rank}{\operatorname*{rank}}
\newcommand{\diag}{\operatorname*{diag}}
\newcommand{\trace}{\operatorname*{trace}}
\newcommand{\sign}{\operatorname*{sign}}
\newcommand{\toep}{\operatorname*{Toep}}
\newcommand{\norm}[1]{\left\lVert{#1}\right\rVert}
\newcommand{\gnorm}[1]{\norm{#1}_{\gamma_2}}
\newcommand{\nnorm}[1]{\norm{#1}_*}
\newcommand{\fnorm}[1]{\norm{#1}_F}
\newcommand{\mrnorm}[1]{\norm{#1}_{2,\infty}}
\newcommand{\ionorm}[1]{\norm{#1}_{\infty,1}}
\newcommand{\dionorm}[1]{\norm{#1}_{\infty,1}^*}

\newcommand{\minimize}{\operatorname*{minimize}}
\newcommand{\maximize}{\operatorname*{maximize}}
\newcommand{\st}{\mbox{subject to}}
\newcommand{\nn}{\nonumber}
\newcommand{\eq}[1]{(\ref{eq:#1})}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\eqdef}{=\vcentcolon}
\newcommand{\Og}{\Omega_{\mathrm{grid}}}
\def \mathbbm {\mathbb}
\def \tmmathbf {\boldsymbol}
\def \tmstrong {\boldsymbol}
\newcommand{\tmop}{\operatorname*}

% Carlos
\newcommand{\cfg}[1]{\textcolor{blue}{#1}}
\newcommand{\bdb}[1]{\textcolor{red}{#1}}
\newcommand{\Id}{\text{\em I}}
\newcommand{\MAT}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\VEC}[1]{\left[\begin{array}{c} #1 \end{array}\right]}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\keys}[1]{\left\{ #1 \right\}}
\newcommand{\sqbr}[1]{\left[ #1 \right]}
\newcommand{\brac}[1]{\left( #1 \right) }
\newcommand{\ml}[1]{\mathcal{ #1 } }
\newcommand{\op}[1]{ \operatorname{#1} }
\newcommand{\normInf}[1]{\left\| #1 \right\| _{\infty}}
\newcommand{\normTwo}[1]{\left\| #1 \right\| _{2}}
\newcommand{\normOne}[1]{\left\| #1 \right\| _{1}}
\newcommand{\normZero}[1]{\left\| #1 \right\| _{0}}
\newcommand{\normTV}[1]{\left\| #1 \right\| _{\op{TV}}}
\newcommand{\normF}[1]{\left\| #1 \right\| _{F}}
\newcommand{\atomicnorm}[1]{\left\| #1 \right| \right|_{\mathcal{A}}}
\newcommand{\der}[2]{\frac{\text{d}#2}{\text{d}#1}}
\newcommand{\derTwo}[2]{\frac{\mathrm{d} ^2#2}{\mathrm{d}#1^2}}
\newcommand{\set}[2]{ \keys{ #1 \; | \; #2 } }
\newcommand{\PROD}[2]{\left \langle #1, #2\right \rangle}
\newcommand{\diff}[1]{ \, \text{d} #1 }
\newcommand{\real}{\op{Re}}
\newcommand{\imag}{\op{Im}}

\newcommand{\signx}{\vct{h}}
\newcommand{\signz}{\vct{r}}

% Constants
\newcommand{\mindisthalf}{1.26}
\newcommand{\mindist}{2.52}
\newcommand{\gammaOne}{0.247}
\newcommand{\gammaTwo}{0.339}
\newcommand{\gammaThree}{0.414}

\newenvironment{Array}{
  \everymath{\displaystyle\everymath{}}
  \setlength\arraycolsep{8pt}
  \def\arraystretch{2}
  \array
}
{
  \endarray
}


==> model.tex <==
\section{Multicompartment Magnetic-Resonance Fingerprinting}

\subsection{Magnetic-resonance fingerprinting}

\cfg{Explanation of the MR fingerprinting model for someone that doesn't know about MRI, ideally with a figure.}

We recently developed a pseudo steady-state free precession (pSSFP) based MRF pulse sequence [22] and a corresponding dictionary simulation and fitting environment that choses the best dictionary atom in the least squares sense [31].

\subsection{Multicompartment model}

\cfg{TO DO: Explanation of the multicompartment model.}

\pgfplotsset{compat = 1.3}
\begin{figure}
\begin{tabular}{ >{\centering\arraybackslash}m{0.55\linewidth}>{\centering\arraybackslash}m{0.3\linewidth}}
\begin{tikzpicture}
\begin{axis}[width=0.65\textwidth, height=0.4\textwidth, xmin=20,xmax=450,ymin=-0.29,ymax=0.1,ticks=none,legend pos=south west]
\addplot[thick,cyan] file {dat_files/single_comp/sig1_single_comp.dat};
\addplot[thick,orange] file {dat_files/single_comp/sig2_single_comp.dat};
\addplot[thick,blue] file {dat_files/single_comp/sig_res_single_comp.dat};
\addplot[thick, red] file {dat_files/single_comp/sig_mix.dat};
\legend{White matter, Myeline, SC model, Data}
\end{axis}
\end{tikzpicture}
&
\begin{tikzpicture}
\begin{axis}[xlabel={$T_1$ (s)}, ylabel={$T_2 $ (s)},legend pos=outer north east, scale=0.75,ylabel shift = 2 pt]
\addplot[scatter, only marks, scatter src=\thisrow{class},scatter/classes={0={mark=square*,cyan}, 1={mark=square*,orange},2={mark=square*,blue}}]
      table[x=x,y=y] {
    x       y        class
    1.0840  0.0690   0
    0.5000  0.0120   1
    0.8557  0.0407   2
};
\end{axis}
\end{tikzpicture}
\end{tabular}
\caption{The left image shows the magnetization signals corresponding to white matter (light blue) and myeline (orange) together with their additive superposition (red), which represents the magnetization data from a voxel with two compartments. A single-compartment (SC) model (blue) is not able to approximate the data (left) and results in an inaccurate estimate of the $T_1$ and $T_2$ parameters (right). The MRF dictionary is generated using the approach in~\cite{asslander2016pseudo}}
\end{figure}



\subsection{Related work}


==> single_voxel_v2.tex <==
\subsection{Single-voxel Simulation}
\label{sec:single_voxel}
We first investigate the performance of the reweighted-$\ell_1$-norm method described in Section~\ref{sec:reweightedl1} on simulated data generated in a single voxel. The ground truth corresponds to two tissues, one of which is fixed to fat ($T_1 = 0.2133$ s and $T_2 = 0.009$ s). The relaxation time of the other compartment varies between $0.1$ s and $2.0$ s for $T_1$ and $0.005$ s and $0.1$ s for $T_2$. The dictionary contains $10609$ logarithmically equal spaced fingerprints in the same $T_1$, $T_2$ range (3\% increment between successive $T_1$ or $T_2$ values). We evaluate for what range of parameters the method achieves recovery. Noise with an i.i.d. Gaussian distribution is added to obtain a signal-to-noise ratio of $100$ or $1000$ (quantified as the ratio between the $\ell_2$ norm of the signal and the noise). Gridding error is induced by setting the true parameters to be randomly located in $T_1$-$T_2$ space, instead of on the discrete values corresponding to fingerprints in the dictionary. \textbf{ST: Do we want to talk about the girding error or we just not mention it?} The reweighted $\ell_1$ algorithm is computed on all these signals using the \textit{sbl} reweighting scheme. \textbf{ST: Do we want to use Candes instead of SBL, since the other numerical experiments in this paper uses Candes as well?}The $\lambda$ hyperparameter is set to $10^{-3}$. 


% TO DO: Description of what sequence this corresponds to and why we chose these parameters






%This experiment is run $5$ times, on a dictionary whose $T_1 ranges \in [.1,2.]$ and $T_2 \in [.005, .1]$. The dictionary has a constant multiplicative factor of $1.03$ between two successive values of $T_1$ as well as $T_2$ and the corresponding number of atoms for each dictionary is then 10609. 

Figure~\ref{fig:sv_experiment} shows is the average of $5$ experiments with the same parameter values. The results plot on the first row show the average number of reconstructed non-zero compartments. The fixed atom (Fat) lies in the middle of the red cross, illustrating that if the two ground truth compartments are very close in $T_1$, $T_2$ space, the algorithm can hardly retrieve the correct number of compartments.

The second row shows the relative error in terms of $T_1$ between the reconstructed atoms and the known ground truth. The relative error is computed by
\begin{equation}
\label{eq:relT1err}
\text{err}_{T_1} = \frac{|\min (\tilde{T}_1) - \min(\hat{T}_1)|}{\min (\tilde{T}_1)} + \frac{|\max (\tilde{T}_1) - \max(\hat{T}_1)|}{\max (\tilde{T}_1)},
\end{equation}
where $\tilde{T}_1$ is a vector containing two ground truth $T_1$ values and $\hat{T}_1$ is a vector of reconstructed $T_1$ values. The third row shows the relative $T_2$ error computed in a similar way:
\begin{equation}
\label{eq:relT2err}
\text{err}_{T_2} = \frac{|\min (\tilde{T}_2) - \min(\hat{T}_2)|}{\min (\tilde{T}_2)} + \frac{|\max (\tilde{T}_2) - \max(\hat{T}_2)|}{\max (\tilde{T}_2)},
\end{equation}
where $\tilde{T}_2$ is the ground truth $T_2$ vector and $\hat{T}_2$ is the reconstructed $T_2$ vector. The second and third row of Figure~\ref{fig:sv_experiment} demonstrates that when two ground truth compartments are too close in their $T_1$, $T_2$ values, the reconstruction error is large due to high correlation between signals. If the two ground truth compartments are fairly far away from each other, the reconstruction results are more accurate. In addition, the range of high error region is larger when the noise level is higher.

\begin{figure}
\label{fig:sv_experiment}
\begin{center}
\begin{tabular}{ >{\centering\arraybackslash}m{0.06\linewidth} >{\centering\arraybackslash}m{0.25\linewidth}  >{\centering\arraybackslash}m{0.25\linewidth} >{\centering\arraybackslash}m{0.25\linewidth} >{\centering\arraybackslash}m{0.02\linewidth} >{\centering\arraybackslash}m{0.02\linewidth}}
& Noiseless & SNR $= 1000$ & SNR $= 100$ & & \\
Non-zero Comp.
&
\includegraphics[width=\linewidth]{asy_pictures/cluster/noiseless/Water/nat_n.pdf}
&
\includegraphics[width=\linewidth]{asy_pictures/cluster/snr1000/l3_s/Water/nat_n.pdf}
&
\includegraphics[width=\linewidth]{asy_pictures/cluster/snr100/l3_s/Water/nat_n.pdf}
&
\includegraphics[height = 2 cm, width = 0.7 cm]{asy_pictures/cluster/bar_nat.png}
&
\includegraphics[height = 2 cm, width = 0.7 cm]{asy_pictures/cluster/bar_nat_lab.png}
\\
$T_1$ Error
&
\includegraphics[width=\linewidth]{asy_pictures/cluster/noiseless/Water/t1_n.pdf}
&
\includegraphics[width=\linewidth]{asy_pictures/cluster/snr1000/l3_s/Water/t1_f.pdf}
&
\includegraphics[width=\linewidth]{asy_pictures/cluster/snr100/l3_s/Water/t1_f.pdf}
&
\includegraphics[height = 2.6 cm, width = 0.7 cm]{asy_pictures/cluster/bar_t1.png}
&
\includegraphics[width = 2 cm]{asy_pictures/cluster/bar_t1_lab.png}
\\
$T_2$ Error
&
\includegraphics[width=\linewidth]{asy_pictures/cluster/noiseless/Water/t2_n.pdf}
&
\includegraphics[width=\linewidth]{asy_pictures/cluster/snr1000/l3_s/Water/t2_f.pdf}
&
\includegraphics[width=\linewidth]{asy_pictures/cluster/snr100/l3_s/Water/t2_f.pdf}
&
\includegraphics[height = 2.6 cm, width = 0.7 cm]{asy_pictures/cluster/bar_t1.png}
&
\includegraphics[width = 2 cm]{asy_pictures/cluster/bar_t2_lab.png}
\end{tabular}
\end{center}
%\caption{Single Voxel reconstruction experiment}
\caption{Single voxel reconstruction experiment corresponds to 50\% of fat ($T_1 = 0.2133$ s and $T_2 = 0.009$ s, marked by a cross) and 50\% of other fingerprints, with $T_1$ between $0.1$ s and $2.0$ s and $T_2$ between $0.005$ s and $0.1$ s. This figure shows the number of non-zero compartments (first row), relative $T_1$ error (second row) and relative $T_2$ error (third row) under different Gaussian noise level. The reconstruction is implemented by the algorithm described in Section~\ref{sec:reweightedl1} and Section~\ref{sec:interior_point}, with regularization parameter $\lambda = 10^{-3}$. Error is computed by Equation~\ref{eq:relT1err} and Equation~\ref{eq:relT2err}.}
\label{fig:noiseless}
\end{figure}

%\begin{tikzpicture}
%\begin{axis}[legend pos=south west, width=0.55\textwidth,height=0.4\textwidth,xmin=25,xmax=70,ticks = none,]
%%xlabel = {t/TR}, 
%% ylabel = {Signal (norm.)}]
%% \addlegendimage{empty legend}
%\addplot[thick,orange] file {dat_files/wm_gm/sig_wm.dat};
%\addplot[thick,cyan] file {dat_files/wm_gm/sig_gm.dat};
%\addplot[thick,blue] file {dat_files/wm_gm/sig_data.dat};
%\addplot[thick,magenta] file {dat_files/wm_gm/sig_sc.dat};
%\legend{White matter, Gray matter, Data, SC model}
%\end{axis}
%\end{tikzpicture}
%\end{tabular}
%\caption{Gray matter and white matter plot. The red rectangle on the left plot is zoomed on the right plot}
%\label{fig:wm_gm}
%\end{figure}

%The problem of deinterlacing the two signals from which the data come from is dependant of the $T_1/T_2$ value of its parameters. The acquisition sequence that was used in the numerical simulations was not built to be able to separate properly tissues like White Matter and Gray Matter. If a voxel would be the sum of these two tissues, the single compartment reconstruction would create a magnetization signal very close to the data coming from the mixture of these two tissues, as can be seen on figure \ref{fig:wm_gm}

